Sample entropy for graph signals: An approach to nonlinear dynamic analysis of data on networks

The recent extension of permutation entropy and its derivatives to graph signals has opened up new horizons for the analysis of complex, high-dimensional systems evolving on networks. However, these measures are all fundamentally rooted in Shannon entropy and symbol dynamics. In this paper, we explore, for the first time, whether and how a popular conditional-entropy based measure --Sample Entropy (SampEn)-- can be effectively defined for graph signals and used to characterise the nonlinear dynamics of data on complex networks. We introduce sample entropy for graph signals (SampEnG), a unified framework that generalises classical sample entropy from uni- and bi-dimensional signals, including time series and images, by building on topology-aware embeddings using multi-hop neighbourhoods and computing finite scale of correlation sums in the continuous embedding state space. Experiments on synthetic and real-world datasets, including weather station, wireless sensor monitoring, and traffic systems, verify that SampEnG recovers known nonlinear dynamical features on paths and grids. In the traffic-flow analysis, SampEnG on a directed topology (encoding causal flow constraint) shows promise to detect phase transitions between free-flow and congestion, offering information that is complementary to existing Shannon-entropy based approaches. We expect SampEnG to open up new ways to analyse graph signals, generalising sample entropy and the concept of conditional entropy to extending nonlinear analysis to a wide variety of network data.

==> supp_tables.tex <==
\begin{table}[t]
\centering
\caption{Robustness of the interior peak (``bend') in the Kuramoto entropy curves, measured by the bend-to-noise ratio $\mathrm{BNR}=[\max_\lambda\overline{E}-\overline{E}(\lambda_{\min})]/\overline{\sigma}_E$ over $M=20$ realisations. $\mathrm{BNR}>1$ indicates the interior rise exceeds the across-realisation noise; $\mathrm{BNR}<1$ indicates it is within noise. A pronounced, robust bend appears only for SampEnG on the RGG.}
\label{tab:supp_bnr}
\begin{tabular}{lcccc}
\toprule
Topology & SampEnG[cos] & SampEnG[sin] & DEG[cos] & DEG[sin] \\
\midrule
RGG & 2.25 & 2.83 & 0.50 & 0.64 \\
ER & 0.11 & 0.52 & 0.02 & 0.09 \\
BA & 0.41 & 0.01 & 0.01 & 0.13 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Projection sensitivity of the Kuramoto entropy curves, measured by the percentage variation of the mean curve across the coupling sweep, $\%\mathrm{var}=100\,(\max\overline{E}-\min\overline{E})/|\overline{E}(\lambda_{\min})|$. A small value indicates the measure is essentially flat across the sweep, i.e.\ unresponsive to the synchronisation transition. DEG[sin] is unresponsive on the ER and BA networks, whereas SampEnG responds on both projections.}
\label{tab:supp_pctvar}
\begin{tabular}{lcccc}
\toprule
Topology & SampEnG[cos] & SampEnG[sin] & DEG[cos] & DEG[sin] \\
\midrule
RGG & 103.4\% & 107.0\% & 44.9\% & 38.7\% \\
ER & 70.4\% & 45.7\% & 26.6\% & 2.0\% \\
BA & 68.8\% & 57.5\% & 26.6\% & 2.2\% \\
\bottomrule
\end{tabular}
\end{table}

